Existence of dissipative solutions to the compressible Navier-Stokes system with potential temperature transport

We introduce dissipative solutions to the compressible Navier-Stokes system with potential temperature transport motivated by the concept of Young measures. We prove their global-in-time existence by means of convergence analysis of a mixed finite element-finite volume method. If a classical solution to the compressible Navier-Stokes system with potential temperature transport exists, we prove the strong convergence of numerical solutions. Our results hold for the full range of adiabatic indices including the physically relevant cases in which the existence of global-in-time weak solutions is open.

==> Commands_old.tex <==
\newtheorem{Theorem}{Theorem}[section]
\newtheorem{Proposition}[Theorem]{Proposition}
\newtheorem{Lemma}[Theorem]{Lemma}
\newtheorem{Corollary}[Theorem]{Corollary}

\theoremstyle{definition}
\newtheorem{Definition}[Theorem]{Definition}


\newtheorem{Example}[Theorem]{Example}
\newtheorem{Remark}[Theorem]{Remark}

\newcommand{\bTheorem}[1]{
\begin{Theorem} \label{T#1} }
\newcommand{\eT}{\end{Theorem}}

\newcommand{\bProposition}[1]{
\begin{Proposition} \label{P#1}}
\newcommand{\eP}{\end{Proposition}}

\newcommand{\bLemma}[1]{
\begin{Lemma} \label{L#1} }
\newcommand{\eL}{\end{Lemma}}

\newcommand{\bCorollary}[1]{
\begin{Corollary} \label{C#1} }
\newcommand{\eC}{\end{Corollary}}

\newcommand{\bRemark}[1]{
\begin{Remark} \label{R#1} }
\newcommand{\eR}{\end{Remark}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\dy}{{\rm d}y}
\newcommand{\Td}{{\mathcal{T}^d}}
\newcommand{\bDefinition}[1]{
\begin{Definition} \label{D#1} }
\newcommand{\eD}{\end{Definition}}
\newcommand{\vve}{\vc{v}_\ep}
\newcommand{\Q}{\mathbb{T}^d}
\newcommand{\toS}{\stackrel{(S)}{\longrightarrow}}
\newcommand{\toSC}{\stackrel{(S)}{\Longrightarrow}}

\newcommand{\Nu}{\mathcal{V}_{t,x}}
\newcommand{\Du}{\mathbb{D}_u}
\newcommand{\DT}{\vc{D}_\vt}
\newcommand{\avg}[1]{ \left< #1 \right>_\Gamma }
\newcommand{\vcg}[1]{{\pmb #1}}
\newcommand{\ave}[1]{ \left< #1 \right>_E }
\newcommand{\avo}[1]{ \left< #1 \right> }
\newcommand{\dif}{\mathrm{d}}
\newcommand{\Del}{\Delta_x}
\newcommand{\rN}{\vr_{h, \mu_n}}
\newcommand{\mN}{\vm_{h, \mu_n}}
\newcommand{\rNN}{\vr_{h_n, \mu_n}}
\newcommand{\mNN}{\vm_{h_n, \mu_n}}

\newcommand{\K}{\mathcal{K}}
\newcommand{\totdif}{\mathrm{D}}
\newcommand{\Pim}{\Pi_{\mathcal{T}}}
\newcommand{\mf}{\mathscr{F}}
\newcommand{\mr}{\mathbb{R}}
\newcommand{\prst}{\mathbb{P}}
% \newcommand{\p}{\mathbb{P}}
\newcommand{\vme}{\vm_\ep}
\newcommand{\eps}{\varepsilon}
\newcommand{\stred}{\mathbb{E}}
\newcommand{\ind}{\mathbf{1}}
\newcommand{\mn}{\mathbb{N}}
\newcommand{\tvU}{\widetilde{\vU}}
\newcommand{\mm}{\mathbb{M}}
\newcommand{\tv}{{\tilde{\vv}}}
\newcommand{\tP}{ {\tilde{\mathbb{P}}}}
\newcommand{\tQ}{{\tilde{\mathbb{Q}}}}
\newcommand{\mt}{\mathbb{T}^N}
\newcommand{\mpi}{\mathrm{\pi}}


\newcommand{\vc}[1]{{\bm #1}}


\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\clo}{cl}
\DeclareMathOperator{\divergence}{div}
\newcommand{\mb}{\mathscr{B}}
\newcommand{\distr}{\overset{d}{\sim}}
\newcommand{\tec}{{\overset{\cdot}{}}}
\newcommand{\semicol}{;}
\newcommand{\data}{{\rm data}}
\newcommand{\bq}{\mathbf q}
\newcommand{\rmk}[1]{\textcolor{red}{#1}}
\newcommand{\bmk}[1]{\textcolor{blue}{#1}}
\newcommand{\jump}[1]{\left[ \!\left[ #1 \right]\! \right]}
\newcommand{\tor}{\mathcal{T}^3}
\newcommand{\tvT}{\tilde{\Theta}}
\newcommand{\StoB}{\left(\Omega, \mathfrak{F},(\mathfrak{F}_t )_{t \geq 0},  \mathbb{P}\right)}
\newcommand{\tvE}{\tilde{E}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfh}{\mathbf{h}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\mE}{\mathcal{E}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\vrh}{\vr_h}
\newcommand{\vrhn}{\vr_{h_n}}
\newcommand{\vmh}{\vm_h}
\newcommand{\vmhn}{\vm_{h_n}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\bfSigma}{\mathbf{\Sigma}}
\newcommand{\bfmu}{\boldsymbol{\mu}}
\newcommand{\bfbeta}{\boldsymbol{\beta}}
\newcommand{\tvm}{\tilde{\vc{m}}}
\newcommand{\bfphi}{\boldsymbol{\varphi}}
\newcommand{\bfvarphi}{\boldsymbol{\varphi}}
\newcommand{\bfPsi}{\boldsymbol{\Psi}}
\newcommand{\bfpsi}{\boldsymbol{\psi}}
\newcommand{\Eh}{E_h}
\newcommand{\BV}{\mathrm{BV}}
%\newcommand{\ds}{\,\mathrm{d}\sigma}
\newcommand{\ds}{\,\mathrm{d}S_x}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\dxs}{\,\mathrm{d}x\,\mathrm{d}\sigma}

\newcommand{\bFormula}[1]{
\begin{equation} \label{#1}}
\newcommand{\eF}{\end{equation}}

\newcommand{\facesint}{\mathcal{E}}
\newcommand{\grid}{\mathcal{T}}
\newcommand{\facesK}{\mathcal{E}(K)}
\newcommand{\vuh}{\vu_h}
\newcommand{\mh}{\vc{m}_h}
\newcommand{\Dh}{\frac{{\rm d}}{{\rm d}t} }
\newcommand{\cD}{c({\rm data}}
\newcommand{\intSh}[1] {\int_{\sigma} #1 \ds }
\newcommand{\TS}{\Delta t}
\newcommand{\bin}{\ \mbox{bounded in}\ }
\newcommand{\The}{\Theta_\ep}
\newcommand{\Divh}{{\rm div}_h}
\newcommand{\Gradh}{\nabla_h}
\newcommand{\Gh}{\Gamma_h}
\newcommand{\Ghi}{\Gamma_{h, {\rm int}}}
\newcommand{\Ghe}{\Gamma_{h, {\rm ext}}}
\newcommand{\co}[2]{{\rm co}\{ #1 , #2 \}}
\newcommand{\Ov}[1]{\overline{#1}}
\newcommand{\av}[1]{ \left\{ #1 \right\}}
\newcommand{\va}[1]{\left<#1\right>}
\newcommand{\Curl}{{\bf curl}_x}
\newcommand{\DC}{C^\infty_c}
\newcommand{\vUm}{\vc{U}_m}
\newcommand{\aleq}{\stackrel{<}{\sim}}

%\newcommand{\toN}{\stackrel{\mathcal{N}}{\to}}
%\newcommand{\toK}{\stackrel{\mathcal{K}}{\to}}
%\newcommand{\toKY}{\stackrel{\mathcal{K}(Y)}{\to}}
%\newcommand{\toWK}{\stackrel{weak-\mathcal{K}}{\to}}
%\newcommand{\toSK}{\stackrel{strong-\mathcal{K}}{\to}}
%\newcommand{\toNY}{\stackrel{\mathcal{N}(Y)}{\to}}
%
\newcommand{\toNY}{\xrightarrow{\mathcal{N}(Y)}}
\newcommand{\toKY}{\xrightarrow{\mathcal{K}(Y)}}
\newcommand{\toWK}{\xrightarrow{weak-\mathcal{K}}}
\newcommand{\toSK}{\xrightarrow{strong-\mathcal{K}}}
\newcommand{\toN}{\xrightarrow{\mathcal{N}}}
\newcommand{\toK}{\xrightarrow{\mathcal{K}}}
%
\newcommand{\ageq}{\stackrel{>}{\sim}}
\newcommand{\Un}[1]{\underline{#1}}
\newcommand{\vr}{\varrho}
\newcommand{\vre}{\vr_\ep}
\newcommand{\Ap}{\Delta_N}
\newcommand{\vte}{\vt_\ep}
\newcommand{\vue}{\vu_\ep}
\newcommand{\tvr}{\tilde \vr}
\newcommand{\tvu}{{\tilde \vu}}
\newcommand{\tvt}{\tilde \vt}
\newcommand{\Dn}{\sqrt{-\Delta_N}}
\newcommand{\vt}{\vartheta}
\newcommand{\vu}{\vc{u}}
\newcommand{\vm}{\vc{m}}
\newcommand{\Ee}{E_{\ep}}
\newcommand{\vM}{\vc{M}}
\newcommand{\vq}{\vc{q}}
\newcommand{\vn}{\vc{n}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\sumK}{\sum_{K \in \grid}}
\newcommand{\sumsf}{\sum_{\sigma \in \faces}}
\newcommand{\sumsfK}{\sum_{\sigma \in \pd K}}
\newcommand\Up{\mbox{\sl{Up}}}
\newcommand{\avs}[1]{\left\{\!\!\left\{ #1\right\}\!\!\right\}}

\newcommand{\muh}{h^\varepsilon}
\newcommand{\ah}{h^{\alpha -1}}

\newcommand{\vvh}{\bm{v}_h}
\newcommand{\pd}{\partial}
\newcommand{\Divup}{{\rm div}_h^{\up}}
\newcommand{\up}{{\rm up}}
\newcommand{\bDhuh}{\bD _h(\vuh)}
\newcommand{\gradd}{\nabla_{\mathcal D}}

\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\bigabs}[1]{\left|#1\right|}
\newcommand{\myangle}[1]{\langle#1\rangle}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\intTd}[1]{\int_{\Td} #1 \, \dx}
\newcommand{\dgrid}{\mathcal{D}_h}
\newcommand{\dgridi}{\mathcal{D}_{i,h}}
\newcommand{\Qh}{Q_h}
\newcommand{\vQh}{\vc{Q}_h}
\newcommand{\Ome}{\Omega_\ep}
\newcommand{\xh}{\vc{x}_h}
\newcommand{\Div}{{\rm div}_x}
\newcommand{\Grad}{\nabla_x}
\newcommand{\Dt}{\frac{\rm d}{{\rm d}t}}
\newcommand{\tn}[1]{\mathbb{#1}}
\newcommand{\dx}{\mathrm{d}\bfx}
\newcommand{\dz}{{\rm d} {z}}
\newcommand{\dt}{\,{\rm d} t }
\newcommand{\iit}{\it}
\newcommand{\ju}[1]{\left[ \left[ #1 \right] \right]}
\newcommand{\trp}[1]{\left( #1 \right)^{\rm out}}
\newcommand{\vU}{\vc{U}}
\newcommand{\Rm}{\mbox{\FF R}}
\newcommand{\dxdt}{\dx\hspace{0.3mm}\dt}
\newcommand{\intO}[1]{\int_{\Td} #1 \ \dx}
\newcommand{\intOO}[1]{\int_{\Ov{\Omega}} #1 \ \dx}
\newcommand{\intQ}[1]{\int_{Q} #1 \ {\rm d}y}
\newcommand{\intOh}[1]{\int_{\Omega_h} #1 \ \dx}
\newcommand{\intK}[1]{\int_{K} #1 \ \dx}
\newcommand{\intE}[1]{\int_E #1 \ \dx}
\newcommand{\intG}[1]{\int_{\Gamma} #1 \ {\rm dS}_x}
\newcommand{\intGE}[1]{\int_{\Gamma_E} #1 \ {\rm dS}_x}
\newcommand{\sumE}{\sum_{E \in E_h}}
\newcommand{\sumG}{\sum_{\Gamma \in \Gamma_h}}
\newcommand{\intOe}[1]{\int_{\Omega_\ep} #1 \ \dx}
\newcommand{\ch}[1]{\textsf{1}_{ #1 } }
\newcommand{\intOB}[1]{\int_{\Omega} \left( #1 \right) \ \dx}
\newcommand{\intRN}[1]{\int_{R^N} #1 \ \dx}
\newcommand{\intR}[1]{\int_{R} #1 \ \dt}
\newcommand{\intRR}[1]{\int_R \int_{R^N} #1 \ \dxdt}
\newcommand{\intTO}[1]{\int_0^T \int_{\Omega} #1 \ \dxdt}
\newcommand{\intTOB}[1]{ \int_0^T \int_{\Omega} \left( #1 \right) \ \dxdt}
\newcommand{\bProof}{{\bf Proof: }}
%\newcommand{\vm}{\vc{v}_m}
\newcommand{\vv}{\vc{v}}
\newcommand{\sumGE}{ \sum_{E \in E_h} \sum_{\Gamma_E \subset \partial E} }
\newcommand{\D}{{\rm d}}
\newcommand{\ep}{\varepsilon}
\newcommand{\bFrame}[1]{\bigskip
             \noindent
                         \begin{tabular}[c] {|p{.96\textwidth}|}  \hline
             \\ #1 \\  \hline \end{tabular}
             \bigskip }
\font\F=msbm10 scaled 1000
\newcommand{\R}{\mathbb{R}}
\newcommand{\I}{\mathbb{I}}
\renewcommand{\S}{\mathbb{S}}
\newcommand{\C}{\mbox{\F C}}
\newcommand{\Cm}{\mbox{\FF C}}
%\newcommand{\E}{\mathbb{E}}
\newcommand{\intTor}[1]{\int_{\mathcal{O}} #1 \ \dx}
\newcommand{\expe}[1]{ \mathbb{E} \left[ #1 \right] }
\newcommand{\bas}{\left\{ \prst, \Omega, \mathfrak{F}, \Big\{ \mathfrak{F}_t \Big\}_{t \geq 0} \right\}}
\newcommand{\DD}{\D^{\rm d}}
\newcommand{\DS}{\D^{\rm s}}
\newcommand{\cred}{\color{red}}
\newcommand{\OOT}{\Omega_{[0,T]}}
\newcommand{\OOI}{\Omega_{[0, \infty)}}
\newcommand{\OTI}{\Omega_{[T, \infty)}}
\newcommand{\POT}{\mathcal{P}_{[0,T]}}
\newcommand{\POI}{\mathcal{P}_{[0, \infty)}}
\newcommand{\PTI}{\mathcal{P}_{[T, \infty)}}
\newcommand{\SOT}{S_{[0,T]}}
\newcommand{\SOI}{S_{[0, \infty)}}
\newcommand{\STI}{S_{[T, \infty)}}
\newcommand{\mathd}{\mathrm{d}}
\newcommand{\tmop}{\text}
% \def\softd{{\leavevmode\setbox1=\hbox{d}%
%           \hbox to 1.05\wd1{d\kern-0.4ex{\char039}\hss}}}

==> Uniqueness.tex <==
The aim of this section is to derive a DMV-strong uniqueness principle for our measure-valued solutions. For this purpose, we rely on the concept of \textit{relative energy}. In view of similar results already available for the Euler system and the compressible Navier-Stokes system -- see \citep[Chapters 6.2 and 6.3]{Feireisl_Lukacova_Book} -- it is convenient to introduce the \textit{total entropy} $S$. It is given by 
\begin{align}
    S = S(\varrho,\theta) = \left\{\begin{array}{cl}
        \varrho\ln\!\left((a\theta^\gamma)^\frac{1}{\gamma-1}\right) & \text{if $\theta >0$,} \\[2mm]
        -\infty & \text{if $\theta=0$}
    \end{array}\right.\,. \label{def_S}
\end{align}
% \begin{align}
%     s = s(\theta) = \left\{\begin{array}{cl}
%         \ln\!\left((a\theta^\gamma)^\frac{1}{\gamma-1}\right) & \text{if $\theta >0$,} \\[2mm]
%         -\infty & \text{if $\theta=0$}
%     \end{array}\right. \qquad \text{and} \qquad S = S(\varrho,\theta) = \varrho s(\theta)\,. \label{def_S}
% \end{align}
Note that the pressure $p=a(\varrho\theta)^\gamma$ can be rewritten with respect to $\varrho$, $S$ as 
\begin{align}
    \p(\varrho,S) = \left\{\begin{array}{cl}
        \varrho^\gamma \exp\left((\gamma-1)\,\dfrac{S}{\varrho}\right) & \text{if $\varrho>0$ and $S\in\reals$,} \\[4mm]
        0 & \text{if $\varrho=0$ and $S\leq 0$, or $S=-\infty$,} \\[2mm]
        \infty & \text{if $\varrho=0$ and $S>0$.}
    \end{array}\right. \label{press_rho_S}
\end{align}
We proceed by defining the relative energy between a triplet of arbitrary smooth functions $(\varrho,\theta,\fatu)$, i.e., 
\begin{align}
    \varrho,\theta\in \Ck{1}(\overline{\Omega}_T)\,, \quad \varrho,\theta>0\,, \quad \fatu\in\Ck{2}(\overline{\Omega}_T)\,, \quad \fatu|_{[0,T]\times\po}=\bm{0}, \label{adm_test_func_rel_energy_inequ}
\end{align}
and a DMV solution $\mathcal{V}$ to the Navier-Stokes system with potential temperature transport (\ref{cequation})--(\ref{isen_press}) in the sense of Definition \ref{def_meas_sol} as
\begin{align}
    E(\mathcal{V}\hspace{0.3mm}|\hspace{0.3mm}\varrho,\theta,\fatu) = \Big\langle\mathcal{V};\frac{1}{2}\,\bvarrho\,|\bfatu-\fatu|^2 + P(\bvarrho,\bS) - \frac{\partial P(\varrho,S)}{\partial \varrho}\,(\bvarrho-\varrho) - \frac{\partial P(\varrho,S)}{\partial S}\,(\bS-S) - P(\varrho,S) \Big\rangle\,, \label{def_rel_energy}
\end{align}
where $P(\varrho,S)=\frac{1}{\gamma-1}\,\p(\varrho,S)$, $S=S(\varrho,\theta)$, and $\bS=S(\bvarrho,\btheta)$. We have the following lemma.

\begin{lemma}[\textbf{Relative energy inequality}]\label{lem_rel_energy_inequ}
Let $(\varrho,\theta,\fatu)$ be a triplet of test functions, cf. $\mathrm{(\ref{adm_test_func_rel_energy_inequ})}$, and $\mathcal{V}$ a DMV solution to $\mathrm{(\ref{cequation})}$--$\mathrm{(\ref{isen_press})}$ in the sense of Definition $\mathrm{\ref{def_meas_sol}}$. Then the relative energy defined in $\mathrm{(\ref{def_rel_energy})}$ satisfies the inequality 
\begin{align}
    &\left[\,\into E(\mathcal{V}_{(t,\,\cdot\,)}\hspace{0.3mm}|\hspace{0.3mm}\varrho,\theta,\fatu)\;\dx\right]_{t\,=\,0}^{t\,=\,\tau} + \int_{\,\overline{\Omega}}\,\dd\mathfrak{E}(\tau) + \int_{\,\overline{\Omega}_\tau}\dd\mathfrak{D} + \inttauinto\mathbb{S}(\gradx(\fatu_\mathcal{V}-\fatu)):\gradx(\fatu_\mathcal{V}-\fatu)\;\dxdt \notag \\[2mm]
    &\quad \leq -\inttauinto \big\langle\mathcal{V};\bvarrho\,(\bfatu-\fatu)^T\cdot\gradx\fatu\cdot(\bfatu-\fatu)\big\rangle\,\dxdt \notag \\[2mm]
    &\quad \phantom{\,\leq\,} -\inttauinto \left\langle\mathcal{V};\p(\bvarrho,\bS) - \frac{\partial \p(\varrho,S)}{\partial \varrho}\,(\bvarrho-\varrho) - \frac{\partial \p(\varrho,S)}{\partial S}\,(\bS-S) - \p(\varrho,S)\right\rangle\divx(\fatu)\;\dxdt \notag \\[2mm]
    &\quad \phantom{\,\leq\,} +\inttauinto \left\langle\mathcal{V};\frac{\bvarrho}{\varrho}\,(\fatu-\bfatu)\right\rangle\cdot\big[\varrho\pt\fatu+\varrho\gradx\fatu\cdot\fatu+\gradx \p(\varrho,S) - \divx(\mathbb{S}(\gradx\fatu))\big]\,\dxdt \notag \\[2mm]
    &\quad \phantom{\,\leq\,} + \inttauinto \left\langle\mathcal{V};(\varrho-\bvarrho\,)\,\frac{1}{\varrho}\,\frac{\partial \p(\varrho,S)}{\partial\varrho}\right\rangle\big[\pt\varrho+\divx(\varrho\fatu)\big]\,\dxdt \notag \\[2mm]
    &\quad \phantom{\,\leq\,} + \inttauinto \left\langle\mathcal{V};(\varrho-\bvarrho\,)\,\frac{1}{\varrho}\,\frac{\partial \p(\varrho,S)}{\partial S}\right\rangle\big[\pt S+\divx(S\fatu)\big]\,\dxdt \notag \\[2mm]
    &\quad \phantom{\,\leq\,} + \inttauinto \left\langle\mathcal{V};\frac{\bvarrho}{\varrho}\,S-\bS\right\rangle\left[\pt\vartheta+\fatu\cdot\gradx\vartheta+\frac{\partial \p(\varrho,S)}{\partial S}\,\divx(\fatu)\right]\dxdt \notag \\[2mm]
    &\quad \phantom{\,\leq\,} +\inttauinto \left\langle\mathcal{V};\left(\frac{\bvarrho}{\varrho}\,S-\bS\right)(\bfatu-\fatu)\right\rangle\cdot\gradx\vartheta\;\dxdt - \inttauinto\gradx\fatu:\dd\bm{\mathfrak{R}}(t)\hspace{0.3mm}\dt \notag \\[2mm]
    &\quad \phantom{\,\leq\,} +\inttauinto \left\langle\mathcal{V};(\bvarrho-\varrho)\,\frac{1}{\varrho}\,\divx(\mathbb{S}(\gradx\fatu))\cdot(\fatu-\bfatu)\right\rangle\dxdt \label{rel_energy_inequ}
\end{align}
for a.a. $\tau\in(0,T)$. Here,
\begin{align*}
    \vartheta = \frac{1}{\gamma-1}\,\frac{\partial \p(\varrho,S)}{\partial S}
\end{align*}
denotes the absolute temperature.
\end{lemma}

\begin{proof}
Using Gauss's theorem we easily verify that
\begin{align*}
    -\inttauinto \mathbb{S}(\gradx\fatu):\gradx(\fatu_\mathcal{V}-\fatu)\;\dxdt &= - \inttauinto \left\langle\mathcal{V};\frac{\bvarrho}{\varrho}\,(\fatu-\bfatu)\right\rangle\cdot\divx(\mathbb{S}(\gradx\fatu))\;\dxdt \notag \\[2mm]
    &\phantom{\,=\,} + \inttauinto \left\langle\mathcal{V};(\bvarrho-\varrho)\,\frac{1}{\varrho}\,\divx(\mathbb{S}(\gradx\fatu))\cdot(\fatu-\bfatu)\right\rangle\dxdt\,.
\end{align*}
Thus, to prove inequality (\ref{rel_energy_inequ}), it suffices to realize that
\begin{align*}
    \left[\,\into E(\mathcal{V}_{(t,\,\cdot\,)}\hspace{0.3mm}|\hspace{0.3mm}\varrho,\theta,\fatu)\;\dx\right]_{t\,=\,0}^{t\,=\,\tau} &= \left[\,\into\left\langle\mathcal{V}_{(t,\,\cdot\,)};\frac{1}{2}\,\bvarrho\,|\bfatu|^2 + P(\bvarrho,\bS)\right\rangle\dx\right]_{t\,=\,0}^{t\,=\tau} + \left[\,\into \p(\varrho,S)\;\dx\right]_{t\,=\,0}^{t\,=\tau} \\[2mm]
    &\phantom{\,=\,}  - \left[\,\into\omean{\mathcal{V}_{(t,\,\cdot\,)};\bS}\,\frac{\partial P(\varrho,S)}{\partial S}\;\dx\right]_{t\,=\,0}^{t\,=\tau} - \left[\,\into\omean{\mathcal{V}_{(t,\,\cdot\,)};\bvarrho\,\bfatu}\cdot\fatu\;\dx\right]_{t\,=\,0}^{t\,=\tau} \\[2mm]
    &\phantom{\,=\,} + \left[\,\into\omean{\mathcal{V}_{(t,\,\cdot\,)};\bvarrho\,}\left(\frac{1}{2}\,|\fatu|^2-\frac{\partial P(\varrho,S)}{\partial\varrho}\right)\dx\right]_{t\,=\,0}^{t\,=\tau}
\end{align*}
and utilize (\ref{energy_inequ})--(\ref{entropy_inequ}) to rewrite the terms on the right-hand side. We omit the necessary computations since they are straightforward and very similar to those leading to \citep[inequality (4.66)]{Feireisl_Lukacova_Book}.
\end{proof}

From the relative energy inequality we can deduce DMV-strong uniqueness.

\begin{corollary}[DMV-strong uniqueness]\label{cor_dmv_strong_uniqueness}
Let the assumptions of Theorem $\mathrm{\ref{thm_main}}$ be satisfied. Further, let $(\varrho,\theta,\fatu)$ be a classical solution to system $\mathrm{(\ref{cequation})}$--$\mathrm{(\ref{isen_press})}$ from the regularity class $\mathrm{(\ref{adm_test_func_rel_energy_inequ})}$ and $\mathcal{V}$ a DMV solution in the sense of Definition $\mathrm{\ref{def_meas_sol}}$ emanating from the same initial data. Then 
\begin{align*}
    \mathfrak{E}=0\,, \quad \mathfrak{D}=0\,, \quad \bm{\mathfrak{R}}=\bm{0}\,, \quad \text{and} \quad \mathcal{V}_{(t,\fatx)}=\delta_{(\varrho(t,\fatx),\theta(t,\fatx),\fatu(t,\fatx))} \quad \text{for a.a. $(t,\fatx)\in\Omega_T$.}
\end{align*}
\end{corollary}

\begin{proof}
Plugging the classical solution $(\varrho,\theta,\fatu)$ into the relative energy inequality (\ref{rel_energy_inequ}), we obtain
\begin{align}
    &\left[\,\into E(\mathcal{V}_{(t,\,\cdot\,)}\hspace{0.3mm}|\hspace{0.3mm}\varrho,\theta,\fatu)\;\dx\right]_{t\,=\,0}^{t\,=\,\tau} + \int_{\,\overline{\Omega}}\,\dd\mathfrak{E}(\tau) + \int_{\,\overline{\Omega}_\tau}\dd\mathfrak{D} + \inttauinto\mathbb{S}(\gradx(\fatu_\mathcal{V}-\fatu)):\gradx(\fatu_\mathcal{V}-\fatu)\;\dxdt \notag \\[2mm]
    &\quad \leq -\inttauinto \big\langle\mathcal{V};\bvarrho\,(\bfatu-\fatu)^T\cdot\gradx\fatu\cdot(\bfatu-\fatu)\big\rangle\,\dxdt \notag \\[2mm]
    &\quad \phantom{\,\leq\,} -\inttauinto \left\langle\mathcal{V};\p(\bvarrho,\bS) - \frac{\partial \p(\varrho,S)}{\partial \varrho}\,(\bvarrho-\varrho) - \frac{\partial \p(\varrho,S)}{\partial S}\,(\bS-S) - \p(\varrho,S)\right\rangle\divx(\fatu)\;\dxdt \notag \\[2mm]
    &\quad \phantom{\,\leq\,} +\inttauinto \left\langle\mathcal{V};\left(\frac{\bvarrho}{\varrho}\,S-\bS\right)(\bfatu-\fatu)\right\rangle\cdot\gradx\vartheta\;\dxdt - \inttauinto\gradx\fatu:\dd\bm{\mathfrak{R}}(t)\hspace{0.3mm}\dt \notag \\[2mm]
    &\quad \phantom{\,\leq\,} +\inttauinto \left\langle\mathcal{V};(\bvarrho-\varrho)\,\frac{1}{\varrho}\,\divx(\mathbb{S}(\gradx\fatu))\cdot(\fatu-\bfatu)\right\rangle\dxdt \notag \\[2mm]
    &\quad \lesssim \inttau\left[\,\into E(\mathcal{V}\hspace{0.3mm}|\hspace{0.3mm}\varrho,\theta,\fatu)\;\dx + \int_{\,\overline{\Omega}}\,\dd\mathfrak{E}(t)\right]\dt +\inttauinto \left\langle\mathcal{V};\left(\frac{\bvarrho}{\varrho}\,S-\bS\right)(\bfatu-\fatu)\right\rangle\cdot\gradx\vartheta\;\dxdt \notag \\[2mm]
    &\quad \phantom{\,\leq\,} +\inttauinto \left\langle\mathcal{V};(\bvarrho-\varrho)\,\frac{1}{\varrho}\,\divx(\mathbb{S}(\gradx\fatu))\cdot(\fatu-\bfatu)\right\rangle\dxdt
    \label{dmv_strong_uniqueness_1}
\end{align}
for a.a. $\tau\in(0,T)$. To handle the last two integrals, we first observe that
\begin{align}
    \inttauinto\mathbb{S}(\gradx(\fatu_\mathcal{V}-\fatu)):\gradx(\fatu_\mathcal{V}-\fatu)\;\dxdt &= \inttauinto\big[\mu|\gradx(\fatu_\mathcal{V}-\fatu)|^2+\nu|\divx(\fatu_\mathcal{V}-\fatu)|^2\big]\,\dxdt \notag \\[2mm]
    &\geq \mu\inttauinto |\gradx(\fatu_\mathcal{V}-\fatu)|^2\;\dxdt\,. \label{dmv_strong_uniqueness_2}
\end{align}
Next, we set
\begin{align*}
    (\underline{\varrho},\overline{\varrho},\underline{\theta},\overline{\theta}) = \left(\inf_{(t,\fatx)\,\in\,\Omega_T}\{\varrho(t,\fatx)\}, \sup_{(t,\fatx)\,\in\,\Omega_T}\{\varrho(t,\fatx)\},\inf_{(t,\fatx)\,\in\,\Omega_T}\{\theta(t,\fatx)\}, \sup_{(t,\fatx)\,\in\,\Omega_T}\{\theta(t,\fatx)\}\right)
\end{align*}
and apply Lemma \ref{aux_lem_rel_energy} to find constants $c_1,c_2,c_3>0$ that only depend on $\underline{\varrho}$, $\overline{\varrho}$, $\underline{\theta}$, $\overline{\theta}$, $c_\star$, and $\gamma$, and corresponding sets
\begin{align*}
    \mathcal{R} &= \left\{(\bvarrho,\btheta,\bfatu)\in\reals^{d+2}\left|\,c_1\underline{\varrho}\leq\bvarrho\leq c_2\overline{\varrho}\,, \; c_\star\leq\btheta \leq c_3\overline{\theta} \right.\right\}, \\[2mm]
    \mathcal{S} &= \left\{(\bvarrho,\btheta,\bfatu)\in\reals^{d+2}\left|\,\bvarrho\geq 0\,, \; \btheta\geq c_\star \right.\right\}\big\backslash \mathcal{R}
\end{align*}
such that 
\begin{align}
    \inttauinto E(\mathcal{V}\hspace{0.3mm}|\hspace{0.3mm}\varrho,\theta,\fatu)\;\dxdt &\gtrsim \inttauinto \big\langle\mathcal{V}; \mathds{1}_\mathcal{R}(\bvarrho,\btheta,\bfatu)\big(|\bfatu-\fatu|^2 + |\bvarrho-\varrho|^2 + |\bS-S|^2\big) \big\rangle\,\dxdt \notag \\[2mm]
    &\phantom{\,\gtrsim\,} +\inttauinto \big\langle\mathcal{V}; \mathds{1}_\mathcal{S}(\bvarrho,\btheta,\bfatu)\big(1+\bvarrho\,|\bfatu-\fatu|^2 + (\bvarrho\btheta)^\gamma\big)\big\rangle\,\dxdt\,. \label{help}
\end{align}
Seeing that
\begin{align*}
    \left|\left(\frac{\bvarrho}{\varrho}\,S-\bS\right)(\bfatu-\fatu)\right| &\lesssim \big|(\bvarrho S -\bS\varrho)(\bfatu-\fatu)\big| \lesssim \big|S(\bvarrho-\varrho)(\bfatu-\fatu)\big| + \big|\varrho(S-\bS)(\bfatu-\fatu)\big| \notag \\[2mm]
    &\lesssim |\bfatu-\fatu|^2 + |\bvarrho-\varrho|^2 + |\bS-S|^2 
\end{align*}
as well as
\begin{align*}
    &\left|\mathds{1}_\mathcal{S}(\bvarrho,\btheta,\bfatu)\left(\frac{\bvarrho}{\varrho}\,S-\bS\right)(\bfatu-\fatu)\right| \notag \\[2mm]
    &\qquad \lesssim \mathds{1}_\mathcal{S}(\bvarrho,\btheta,\bfatu)\left(\bvarrho\,|\bfatu-\fatu| + \bS\,|\bfatu-\fatu|\right) \lesssim \mathds{1}_\mathcal{S}(\bvarrho,\btheta,\bfatu)\left(\bvarrho\,|\bfatu-\fatu| + \bvarrho\btheta^{\,1/2}\,|\bfatu-\fatu|\right) \notag \\[2mm]
    &\qquad \lesssim \mathds{1}_\mathcal{S}(\bvarrho,\btheta,\bfatu)\left(\bvarrho + \bvarrho\btheta + \bvarrho\,|\bfatu-\fatu|^2\right) \lesssim \mathds{1}_\mathcal{S}(\bvarrho,\btheta,\bfatu)\left(1 + \bvarrho\,|\bfatu-\fatu|^2 + (\bvarrho\btheta)^\gamma\right),
\end{align*}
we may use (\ref{help}) to deduce 
\begin{align}
    \left|\,\inttauinto \left\langle\mathcal{V};\left(\frac{\bvarrho}{\varrho}\,S-\bS\right)(\bfatu-\fatu)\right\rangle\cdot\gradx\vartheta\;\dxdt\,\right| \lesssim \inttauinto E(\mathcal{V}\hspace{0.3mm}|\hspace{0.3mm}\varrho,\theta,\fatu)\;\dxdt\,. \label{dmv_strong_uniqueness_3}
\end{align}
We proceed by observing that
\begin{align*}
    \big|(\bvarrho-\varrho)(\fatu-\bfatu)\big| \lesssim |\bvarrho-\varrho|^2 + |\bfatu-\fatu|^2
\end{align*}
and 
\begin{align*}
    \big|\mathds{1}_\mathcal{S}(\bvarrho,\btheta,\bfatu)(\bvarrho-\varrho)(\fatu-\bfatu)\big| &\lesssim \mathds{1}_\mathcal{S}(\bvarrho,\btheta,\bfatu)(\bvarrho+1)|\bfatu-\fatu| \notag \\[2mm]
    &\lesssim \mathds{1}_\mathcal{S}(\bvarrho,\btheta,\bfatu)\left(\bvarrho + \bvarrho\,|\bfatu-\fatu|^2 + \alpha|\bfatu-\fatu|^2 + \alpha^{-1}\right) \notag \\[2mm]
    &\lesssim \mathds{1}_\mathcal{S}(\bvarrho,\btheta,\bfatu)\left(1+(\bvarrho\btheta)^\gamma + \bvarrho\,|\bfatu-\fatu|^2 + \alpha|\bfatu-\fatu|^2 + \alpha^{-1}\right)
\end{align*}
for all $\alpha>0$, where here and in the sequel the constant hidden in "$\lesssim$" does not depend on $\alpha$. Together with (\ref{help}) and (\ref{poincare_inequ}), these observations yield
\begin{align}
    &\left|\,\inttauinto \left\langle\mathcal{V};(\bvarrho-\varrho)\,\frac{1}{\varrho}\,\divx(\mathbb{S}(\gradx\fatu))\cdot(\fatu-\bfatu)\right\rangle\dxdt\,\right| \notag \\[2mm]
    &\lesssim (1+\alpha^{-1}) \inttauinto E(\mathcal{V}\hspace{0.3mm}|\hspace{0.3mm}\varrho,\theta,\fatu)\;\dxdt + \alpha\left(\,\inttauinto|\gradx(\fatu_{\mathcal{V}}-\bm{u})|^2\;\dxdt+ \inttau\!\!\int_{\,\overline{\Omega}}\,\dd\mathfrak{E}(t)\hspace{0.3mm}\dt + \int_{\,\overline{\Omega}_\tau}\!\dd\mathfrak{D}\right)\,. \label{dmv_strong_uniqueness_4}
\end{align}
Finally, combining (\ref{dmv_strong_uniqueness_1}), (\ref{dmv_strong_uniqueness_2}), (\ref{dmv_strong_uniqueness_3}), and (\ref{dmv_strong_uniqueness_4}), we arrive at
\begin{align*}
    &\left[\,\into E(\mathcal{V}_{(t,\,\cdot\,)}\hspace{0.3mm}|\hspace{0.3mm}\varrho,\theta,\fatu)\;\dx\right]_{t\,=\,0}^{t\,=\,\tau} + \int_{\,\overline{\Omega}}\,\dd\mathfrak{E}(\tau) + \int_{\,\overline{\Omega}_\tau}\dd\mathfrak{D} + \mu\inttauinto |\gradx(\fatu_\mathcal{V}-\fatu)|^2\;\dxdt \notag \\[2mm]
    &\quad \lesssim (1+\alpha^{-1}) \inttauinto E(\mathcal{V}\hspace{0.3mm}|\hspace{0.3mm}\varrho,\theta,\fatu)\;\dxdt + (1+\alpha)\inttau\!\!\int_{\,\overline{\Omega}}\,\dd\mathfrak{E}(t)\hspace{0.3mm}\dt \notag \\[2mm]
    &\quad \phantom{\,\lesssim\,} +\alpha\left(\,\inttauinto|\gradx(\fatu_{\mathcal{V}}-\bm{u})|^2\;\dxdt + \int_{\,\overline{\Omega}_\tau}\!\dd\mathfrak{D}\right)
\end{align*}
for a.a. $\tau\in(0,T)$ and all $\alpha>0$. In particular, there exists a constant $C>0$ such that 
\begin{align*}
    &\left[\,\into E(\mathcal{V}_{(t,\,\cdot\,)}\hspace{0.3mm}|\hspace{0.3mm}\varrho,\theta,\fatu)\;\dx\right]_{t\,=\,0}^{t\,=\,\tau} + \int_{\,\overline{\Omega}}\,\dd\mathfrak{E}(\tau) + \int_{\,\overline{\Omega}_\tau}\dd\mathfrak{D} \notag \\[2mm]
    &\qquad\qquad\qquad \leq C\left(\,\inttauinto E(\mathcal{V}\hspace{0.3mm}|\hspace{0.3mm}\varrho,\theta,\fatu)\;\dxdt + \inttau\!\!\int_{\,\overline{\Omega}}\,\dd\mathfrak{E}(t)\hspace{0.3mm}\dt + \inttau\!\!\int_{\,\overline{\Omega}_t}\dd\mathfrak{D}\hspace{0.3mm}\dt\right)
\end{align*}
for a.a. $\tau\in(0,T)$. Consequently, the desired result follows from Gronwall's inequality.
\end{proof}

\begin{corollary}\label{cor_strong_conv}
Let the assumptions of Theorem $\mathrm{\ref{thm_main}}$ be satisfied and suppose there is a classical solution $(\varrho,\theta,\fatu)$ to system $\mathrm{(\ref{cequation})}$--$\mathrm{(\ref{isen_press})}$ from the regularity class $\mathrm{(\ref{adm_test_func_rel_energy_inequ})}$ emanating from the chosen initial data. Further, let $(\varrho_h,\thetah,\fatu_h)_{h\,\downarrow\,0}$ be a sequence of solutions to the FE-FV method $\mathrm{(\ref{r_method})}$--$\mathrm{(\ref{m_method})}$ starting from the corresponding discrete initial data defined in $\mathrm{(\ref{disc_int_1})}$ and suppose the parameters satisfy $\mathrm{(\ref{cons_cond})}$. Then
\begin{align*}
    \varrho_h \rightarrow \varrho \;\;\text{in $\Lp{\gamma}{0mm}(\Omega_T)$,} \quad \thetah\rightarrow\theta \;\; \text{in $\Lp{p}{0.5mm}(\Omega_T)$ for all $p\in[1,\infty)$,} \quad \text{and} \quad \fatu_h\rightarrow\fatu \;\; \text{in $\Lp{2}{0mm}(\Omega_T)^d$} 
\end{align*}
as $h\downarrow 0$.
\end{corollary}

\begin{proof}
Let $(\varrho_h,\thetah,\fatu_h)_{h\,\downarrow\,0}$ be a sequence as described above. To prove Corollary \ref{cor_strong_conv}, it suffices to show that every subsequence $(\varrho_i,\theta_i,\fatu_i)_{i\,\downarrow\,0}$ of $(\varrho_h,\thetah,\fatu_h)_{h\,\downarrow\,0}$ possesses a subsequence $(\varrho_\ell,\theta_\ell,\fatu_\ell)_{\ell\,\downarrow\,0}$ such that
\begin{align*}
    \varrho_\ell \rightarrow \varrho \;\;\text{in $\Lp{\gamma}{0mm}(\Omega_T)$,} \quad \theta_\ell\rightarrow\theta \;\; \text{in $\Lp{p}{0.5mm}(\Omega_T)$ for all $p\in[1,\infty)$,} \quad \text{and} \quad \fatu_\ell\rightarrow\fatu \;\; \text{in $\Lp{2}{0mm}(\Omega_T)^d$} 
\end{align*}
as $\ell\downarrow 0$. Thus, let $(\varrho_i,\theta_i,\fatu_i)_{i\,\downarrow\,0}$ be an arbitrary subsequence of $(\varrho_h,\thetah,\fatu_h)_{h\,\downarrow\,0}$. From the proof of Theorem \ref{thm_main} and the DMV-strong uniqueness principle established in the previous corollary we deduce that there is a subsequence $(\varrho_j,\theta_j,\fatu_j)_{j\,\downarrow\,0}$ of $(\varrho_i,\theta_i,\fatu_i)_{i\,\downarrow\,0}$ such that
\begin{gather*}
    \varrho_j\theta_j^m \rightharpoonup \varrho\theta^m \;\;\text{in $\Lp{\gamma}{0mm}(\Omega_T)$ for all $m\in\naturals_0$,} \qquad \varrho_j\theta_j \to \varrho\theta \;\;\text{in $\Lp{\gamma}{0mm}(\Omega_T)$,} \\[2mm]
    \varrho_j\overline{\fatu_j} \rightharpoonup \varrho\fatu \;\;\text{in $\Lp{\tfrac{2\gamma}{\gamma+1}}{0mm}(\Omega_T)^d$,} \qquad \fatu_j \rightharpoonup \fatu \;\;\text{in $\Lp{2}{0mm}(\Omega_T)^d$,} \\[2mm]
    \gradh\fatu_j \rightharpoonup \gradx\fatu \;\;\text{in $\Lp{2}{0mm}(\Omega_T)^{d\times d}$,} \qquad \text{and} \qquad \lnorm{\varrho_j|\overline{\fatu_j}|^2}{1}{(\Omega_T)}{0.55}{-0.5mm} \to \lnorm{\varrho|\fatu|^2}{1}{(\Omega_T)}{0.55}{-0.5mm}
\end{gather*}
as $j\downarrow 0$. Consequently,
\begin{align*}
    \lnorm{\varrho_j-\varrho}{1}{(\Omega_T)}{0.55}{-0.5mm} &\lesssim \lnorm{\varrho_j\theta-\varrho\theta}{1}{(\Omega_T)}{0.55}{-0.5mm} \lesssim \lnorm{\varrho_j\theta_j-\varrho\theta}{1}{(\Omega_T)}{0.55}{-0.5mm} + \lnorm{\varrho_j\theta-\varrho_j\theta_j}{1}{(\Omega_T)}{0.55}{-0.5mm} \notag \\[2mm]
    &\lesssim \lnorm{\varrho_j\theta_j-\varrho\theta}{\gamma}{(\Omega_T)}{0.55}{-0.5mm} + \left(\lnorm{\varrho_j}{1}{(\Omega_T)}{0.55}{-0.5mm}\,\lnorm{\varrho_j(\theta-\theta_j)^2}{1}{(\Omega_T)}{0.55}{-0.5mm}\right)^{1/2} \notag \\[2mm]
    &\lesssim \lnorm{\varrho_j\theta_j-\varrho\theta}{\gamma}{(\Omega_T)}{0.55}{-0.5mm} + \explnorm{\varrho_j(\theta-\theta_j)^2}{1}{(\Omega_T)}{0.55}{-0.5mm}{0.5mm}{1/2} \xrightarrow{\,j\,\downarrow\,0\,} 0\,,
\end{align*}
i.e., $\varrho_j\to\varrho$ in $\Lp{1}{0mm}(\Omega_T)$ as $j\downarrow 0$. Moreover, there is a subsequence $(\varrho_\ell,\theta_\ell,\fatu_\ell)_{\ell\,\downarrow\,0}$ of $(\varrho_j,\theta_j,\fatu_j)_{j\,\downarrow\,0}$ such that $\varrho_\ell\to\varrho$ in $\Lp{\gamma}{0mm}(\Omega_T)$. Therefore,
\begin{align*}
    \lnorm{(\fatu_\ell-\fatu)^{2}}{1}{(\Omega_T)}{0.55}{-0.5mm} &\lesssim \lnorm{(\fatu_\ell-\overline{\fatu_\ell})^{2}}{1}{(\Omega_T)}{0.55}{-0.5mm} + \lnorm{(\overline{\fatu_\ell}-\fatu)^{2}}{1}{(\Omega_T)}{0.55}{-0.5mm} \\[2mm]
    &\lesssim h^2\,\explnorm{\gradh\fatu_\ell}{2}{(\Omega_T)^{d\times d}}{0.55}{-0.5mm}{0.5mm}{2} + \lnorm{(\overline{\fatu_\ell}-\fatu)^{2}}{1}{(\Omega_T)}{0.55}{-0.5mm} \\[2mm]
    &\lesssim h^2 + \lnorm{\mathds{1}_{\{\varrho_\ell\,\leq\, \underline{\varrho}/2\}}(\overline{\fatu_\ell}-\fatu)^{2}}{1}{(\Omega_T)}{0.55}{-0.5mm} + \lnorm{\varrho_\ell(\overline{\fatu_\ell}-\fatu)^{2}}{1}{(\Omega_T)}{0.55}{-0.5mm} \xrightarrow{\,\ell\,\downarrow\,0\,} 0\,, \\[2mm]
    \lnorm{(\theta_\ell-\theta)^{2m}}{1}{(\Omega_T)}{0.55}{-0.5mm} &\lesssim \lnorm{\mathds{1}_{\{\varrho_\ell\,\leq\, \underline{\varrho}/2\}}(\theta_\ell-\theta)^{2m}}{1}{(\Omega_T)}{0.55}{-0.5mm} + \lnorm{\varrho_\ell(\theta_\ell-\theta)^{2m}}{1}{(\Omega_T)}{0.55}{-0.5mm} \xrightarrow{\,\ell\,\downarrow\,0\,} 0
\end{align*}
for all $m\in\naturals$, where $\underline{\varrho}=\inf_{(t,\fatx)\,\in\,\Omega_T}\{\varrho(t,\fatx)\}>0$. In particular, $\fatu_\ell\to\fatu$ in $\Lp{2}{0mm}(\Omega_T)^d$ and $\theta_\ell\to\theta$ in $\Lp{p}{0.5mm}(\Omega_T)$ for all $p\in[1,\infty)$ as $\ell\downarrow 0$. 
\end{proof}
